II-MMR: Identifying and Improving Multi-modal Multi-hop Reasoning in Visual Question Answering

Visual Question Answering (VQA) often involves diverse reasoning scenarios across Vision and Language (V&L). Most prior VQA studies, however, have merely focused on assessing the model's overall accuracy without evaluating it on different reasoning cases. Furthermore, some recent works observe that conventional Chain-of-Thought (CoT) prompting fails to generate effective reasoning for VQA, especially for complex scenarios requiring multi-hop reasoning. In this paper, we propose II-MMR, a novel idea to identify and improve multi-modal multi-hop reasoning in VQA. In specific, II-MMR takes a VQA question with an image and finds a reasoning path to reach its answer using two novel language promptings: (i) answer prediction-guided CoT prompt, or (ii) knowledge triplet-guided prompt. II-MMR then analyzes this path to identify different reasoning cases in current VQA benchmarks by estimating how many hops and what types (i.e., visual or beyond-visual) of reasoning are required to answer the question. On popular benchmarks including GQA and A-OKVQA, II-MMR observes that most of their VQA questions are easy to answer, simply demanding "single-hop" reasoning, whereas only a few questions require "multi-hop" reasoning. Moreover, while the recent V&L model struggles with such complex multi-hop reasoning questions even using the traditional CoT method, II-MMR shows its effectiveness across all reasoning cases in both zero-shot and fine-tuning settings.

==> todo.tex <==
\section{TODO}
\begin{itemize} [itemsep=0pt,topsep=0.0pt,leftmargin=10pt,partopsep=0pt]
    \item human evaluation for the quality of our rationales
    \item change figures: (1) Non-visual --> Beyond-visual, (2) captions, (3) maybe combine \apcot and \ktprompt into figure2
    
    %\item Org+Aug in Table 11 (LLaMA2 13B or 70B)
    
    %\item Direct LLM prompting for augmentation
    %\item STaR: Bootstrapping Reasoning With Reasoning
    %\item In-context learning (GPT4-V or LLaVA1.5)
    
\end{itemize}
